RecSys-DAN: Discriminative Adversarial Networks for Cross-Domain Recommender Systems

Data sparsity and data imbalance are practical and challenging issues in cross-domain recommender systems. This paper addresses those problems by leveraging the concepts which derive from representation learning, adversarial learning and transfer learning (particularly, domain adaptation). Although various transfer learning methods have shown promising performance in this context, our proposed novel method RecSys-DAN focuses on alleviating the cross-domain and within-domain data sparsity and data imbalance and learns transferable latent representations for users, items and their interactions. Different from existing approaches, the proposed method transfers the latent representations from a source domain to a target domain in an adversarial way. The mapping functions in the target domain are learned by playing a min-max game with an adversarial loss, aiming to generate domain indistinguishable representations for a discriminator. Four neural architectural instances of ResSys-DAN are proposed and explored. Empirical results on real-world Amazon data show that, even without using labeled data (i.e., ratings) in the target domain, RecSys-DAN achieves competitive performance as compared to the state-of-the-art supervised methods. More importantly, RecSys-DAN is highly flexible to both unimodal and multimodal scenarios, and thus it is more robust to the cold-start recommendation which is difficult for previous methods.

==> Conclusion.tex <==
%!TEX root = Main.tex
\section{Conclusion}
\label{sec:con}

RecSys-DAN is a novel framework for cross-domain collaborative filtering,
particularly, the real-world cold-start recommendation problem. It learns to
adapt the user, item and user-item interaction representations from a source
domain to a target domain in an unsupervised and adversarial fashion.
Multiple generators and discriminators are designed to adversarially learn
target generators for generating domain-invariant representations. Four
RecSys-DAN instances, namely, UI-DAN, U-DAN, I-DAN, and H-DAN, are explored
by considering different scenarios characterized by the overlap of users and
items in both unimodal and multimodal settings. Experimental results
demonstrates that RecSys-DAN has a competitive performance compared to
state-of-the-art supervised methods for the rating prediction task, even with
absent preference information.
